Implicational Relevance Logic is 2-EXPTIME-Complete

We show that provability in the implicational fragment of relevance logic is complete for doubly exponential time, using reductions to and from coverability in branching vector addition systems.

==> proof-cl-exp-fl2.tex <==
  

